Moduli Spaces of Sheaves on General Blow-ups of $\mathbb{P}^2$

Let $X$ be the blow-up of $\mathbb{P}^2$ along $m$ general points, and $A=H-\sum \varepsilon_iE_i$ be a generic polarization with $0<\varepsilon_i\ll1$. We classify the Chern characters which satisfy the weak Brill-Noether property, i.e. a general sheaf in $M_A({\bf{v}})$, the moduli space of slope stable sheaves with Chern character ${\bf{v}}$, has at most one non-zero cohomology. We further give a necessary and sufficient condition for the existence of stable sheaves. Our strategy is to specialize to the case when the $m$ points are collinear.

==> citation.tex <==



@article{ABCH13,
  title={The minimal model program for the \textup{Hilbert} scheme of points on $\mb{P}^2$ and Bridgeland stability},
  author={Arcara, Daniele and Bertram, Aaron and Coskun, Izzet and Huizenga, Jack},
  journal={Advances in mathematics},
  volume={235},
  pages={580--626},
  year={2013},
  publisher={Elsevier}
}


@article{LQZ03,
  title={\textup{Curves in the Hilbert schemes of points on surfaces}},
  author={W-P Li and Z Qin and Q Zhang},
  journal={Contemporary Mathematics},
  volume={322},
  pages={89--96},
  year={2003},
  publisher={Providence, RI; American Mathematical Society; 1999}
}

@article{Muk87,
  title={\textup{On the moduli space of bundles on K3 surfaces. I}},
  author={Mukai, Shigeru},
  journal={Vector bundles on algebraic varieties (Bombay, 1984)},
  volume={11},
  pages={341--413},
  year={1984}
}



@article{Hui16,
  title={\textup{Effective divisors on the Hilbert scheme of points in the plane and interpolation for stable bundles}},
  author={Huizenga, Jack},
  journal={J. Algebraic Geom.},
  volume={25},
  pages={19-75},
  year={2016},
  publisher={Elsevier}
}


@article{Rud94,
  title={\textup{A description of Chern classes of semistable sheaves on a quadric surface}},
  author={Rudakov, Alexei N},
  journal={J. reine angew. Math.},
  volume={453},
  pages={113–135},
  year={1994},
}


@article{BB,
  title={\textup{Nef cones of Hilbert schemes of points on surfaces}},
  author={Bolognese, Barbara and Huizenga, Jack and Lin, Yinbang and Riedl, Eric and Schmidt, Benjamin and Woolf, Matthew and Zhao, Xiaolei},
  journal={Algebra \& Number Theory},
  volume={10},
  number={4},
  pages={907--930},
  year={2016},
  publisher={Mathematical Sciences Publishers}
}


@incollection{BC13,
  title={\textup{The birational geometry of the Hilbert scheme of points on surfaces}},
  author={Bertram, Aaron and Coskun, Izzet},
  booktitle={Birational geometry, rational curves, and arithmetic},
  pages={15--55},
  year={2013},
  publisher={Springer}
}

@incollection{BS88,
  title={On k-spannedness for projective surfaces},
  author={Beltrametti, Mauro and Sommese, Andrew J},
  booktitle={Algebraic geometry},
  pages={24--51},
  year={1988},
  publisher={Springer}
}



@article{CH20,
  title={{B}rill-{N}oether theorems and globally generated vector bundles on {H}irzebruch surfaces},
  author={Coskun, Izzet and Huizenga, Jack},
  journal={Nagoya Mathematical Journal},
  volume={238},
  pages={1--36},
  year={2020},
  publisher={Cambridge University Press}
}


@article{CH16,
  title={Weak {B}rill-{N}oether for rational surfaces},
  author={Coskun, Izzet and Huizenga, Jack},
  journal={Local and Global Methods in Algebraic Geometry, Contemporary Mathematics},
  volume={712},
  pages={81--104},
  year={2018},
}


@article{CHW17,
  title={The effective cone of the moduli space of sheaves on the plane},
  author={Coskun, Izzet and Huizenga, Jack and Woolf, Matthew},
  journal={Journal of the European Mathematical Society},
  volume={19},
  number={5},
  pages={1421--1467},
  year={2017}
}

@article{CH18,
  title={The nef cone of the moduli space of sheaves and strong {B}ogomolov inequalities},
  author={Coskun, Izzet and Huizenga, Jack},
  journal={Israel Journal of Mathematics},
  volume={226},
  number={1},
  pages={205--236},
  year={2018},
  publisher={Springer}
}


@article{CH21,
  title={Existence of semistable sheaves on {H}irzebruch surfaces},
  author={Coskun, Izzet and Huizenga, Jack},
  journal={Advances in Mathematics},
  volume={381},
  year={2021},
  publisher={Elsevier}
}




@inproceedings{DLP85,
  title={Fibr{\'e}s stables et fibr{\'e}s exceptionnels sur $\mb{P}^2$},
  author={Dr\'{e}zet, J-M and Le Potier, Joseph},
  booktitle={Annales scientifiques de l'{\'E}cole Normale Sup{\'e}rieure},
  volume={18},
  number={2},
  pages={193--243},
  year={1985}
}


@article{Fog73,
  title={Algebraic families on an algebraic surface, {II}, the {P}icard scheme of the punctual {H}ilbert scheme},
  author={Fogarty, John},
  journal={American Journal of Mathematics},
  volume={95},
  number={3},
  pages={660--687},
  year={1973},
  publisher={JSTOR}
}





@article{GH98,
  title={Weak {B}rill-{N}oether for vector bundles on the projective plane},
  author={G\"{o}ttsche, Lothar and Hirschowitz, Andr\'{e}},
   journal={Algebraic
   geometry \textup{(Catania, 1993/Barcelona, 1994), 63–74}, Lecture Notes in Pure and Appl. Math., \textup{200} Dekker,
New York},
   year={1994},
}





@book{Har77,
  title={Algebraic {G}eometry},
  author={Hartshorne, Robin},
  journal={Graduate texts in mathematics},
  volume={52},
  year={1977},
  publisher={Springer}
}

@book{Har10,
  title={Deformation {T}heory},
  author={Hartshorne, Robin},
  journal={Graduate texts in mathematics},
  volume={257},
  year={2010},
  publisher={Springer}
}




@book{HL10,
  title={The geometry of moduli spaces of sheaves},
  author={Huybrechts, Daniel and Lehn, Manfred},
  year={2010},
  publisher={Cambridge University Press}
}



@article{KO95,
  title={Exceptional sheaves on del {P}ezzo surfaces},
  author={Kuleshov, SA and Orlov, Dmitri Olegovich},
  journal={Izvestiya: Mathematics},
  volume={44},
  number={3},
  pages={479},
  year={1995},
  publisher={IOP Publishing}
}


@book{Lar04,
  title={Positivity in algebraic geometry {I}: {C}lassical setting: line bundles and linear series},
  author={Lazarsfeld, Robert K},
  volume={48},
  year={2004},
  publisher={Springer}
}


@book{LeP97,
  title={Lectures on vector bundles},
  author={Le Potier, Joseph},
  year={1997},
  publisher={Cambridge University Press}
}


@article{LZ19,
  title={Brill-{N}oether and existence of semistable sheaves for del {P}ezzo surfaces, submitted preprint},
  author={Levine, D and Zhang, S},
  year={2019},
}



@article{Wal95,
  title={Components of the stack of torsion-free sheaves of rank 2 on ruled surfaces},
  author={Walter, Charles H},
  journal={Math. Ann.},
  volume={301(4)},
  pages={699--715},
  year={1995},
}





@article{Wal98,
  title={Irreducibility of moduli spaces of vector bundles on birationally ruled surfaces},
  author={Walter, Charles},
   journal={Algebraic
   geometry \textup{(Catania, 1993/Barcelona, 1994)}, Lecture Notes in Pure and Appl. Math., \textup{200}},
   pages={201--211},
   year={1998},
}


